Cooperative Resilience in Artificial Intelligence Multiagent Systems

Resilience refers to the ability of systems to withstand, adapt to, and recover from disruptive events. While studies on resilience have attracted significant attention across various research domains, the precise definition of this concept within the field of cooperative artificial intelligence remains unclear. This paper addresses this gap by proposing a clear definition of `cooperative resilience' and outlining a methodology for its quantitative measurement. The methodology is validated in an environment with RL-based and LLM-augmented autonomous agents, subjected to environmental changes and the introduction of agents with unsustainable behaviors. These events are parameterized to create various scenarios for measuring cooperative resilience. The results highlight the crucial role of resilience metrics in analyzing how the collective system prepares for, resists, recovers from, sustains well-being, and transforms in the face of disruptions. These findings provide foundational insights into the definition, measurement, and preliminary analysis of cooperative resilience, offering significant implications for the broader field of AI. Moreover, the methodology and metrics developed here can be adapted to a wide range of AI applications, enhancing the reliability and effectiveness of AI in dynamic and unpredictable environments.

==> sections/impact.tex <==
This paper introduces a consolidated definition and quantitative measurement of `Cooperative resilience' in artificial intelligence systems. By analyzing how RL-based and LLM-based autonomous agents respond to disruptive events, such as environmental changes and unsustainable behaviors, within a simulated social dilemma, we highlight the critical importance of resilience metrics. Our findings provide a framework for understanding how cooperative AI systems prepare for, resist, recover from, and adapt to disruptions. This work is poised to influence the development of more robust cooperative AI systems, particularly in domains where complex agent interactions and dynamic environments can lead to vulnerabilities and unpredictable failures. Besides, the introduction of resilience metrics lays the foundation for regulatory frameworks, ensuring that AI systems deployed in critical sectors are both intelligent and resilient, ultimately contributing to societal stability and well-being.
